Model-Free Output Tracking of Nonlinear Systems via High-Frequency Dither

This paper investigates model-free output tracking of time-varying reference trajectories for a class of unknown nonlinear control-affine systems with known relative degree one. The tracking problem is formulated as the minimisation of a time-varying objective function, and a high-frequency-dither-based controller is developed using only measured output performance, without requiring knowledge of the plant dynamics or control direction. By deliberately introducing high-frequency excitation, the proposed approach establishes an exploitable separation of time scales. A coordinate transformation inspired by vibrational control removes the explicit high-frequency input term, enabling partial averaging of the nonlinear closed-loop dynamics. For analysis, the partial averaging step reveals an effective gradient-descent-like tracking mechanism whose stabilising action is independent of the sign of the unknown input-output gain. Under suitable assumptions on the internal dynamics, semiglobal practical exponential convergence guarantees on the tracking of time-varying reference trajectories is established for appropriately selected controller parameters and sufficiently high dither frequencies. While sharing the optimisation-based perspective of extremum-seeking control, the proposed approach addresses time-varying optimisation in the presence of unknown nonlinear plant dynamics without relying on an input to steady-state output mapping. By exploiting transient plant dynamics through high-frequency excitation, the proposed framework provides a foundation for extending the approach to more general time-varying performance objectives and incorporating input and output constraints.

==> Chapters/Main_Result_Backup.tex <==



\subsection{Controller Design}
We formulate the tracking task using the time-varying objective
\begin{equation}
    J(t,y)\coloneqq\big(y-y_d(t)\big)^2.
    \label{eq:tracking_objective}
\end{equation}
The measured output and the reference are available for evaluating
\eqref{eq:tracking_objective}.

We consider the extremum-seeking controller shown in
Figure~\ref{fig:block_diagram}:
\begin{equation}
    \label{eq:control_law}
    \begin{aligned}
        \dot{\hat v}
        &=-KJ(t,y)\sin(\omega t),\\
        v&=\hat v+a\sin(\omega t),\\
        u&=\dot v+\lambda v,
    \end{aligned}
\end{equation}
where $a>0$ is the dither amplitude, $\omega>0$ is the dither frequency, and $K,\lambda>0$ are controller gains.
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures/Block_diagram.pdf}
    \caption{Block diagram of the output tracking controller.}
    \label{fig:block_diagram}
\end{figure}

By \eqref{eq:control_law}, the input can be evaluated as
\begin{equation}
    \begin{aligned}
        u
        ={}&-KJ(t,y)\sin(\omega t) +a\omega\cos(\omega t)+\lambda\hat v+\lambda a\sin(\omega t).
    \end{aligned}
    \label{eq:control_input_explicit}
\end{equation}
Thus, implementation does not require numerical differentiation of the measured output.

The resulting closed-loop system is
\begin{equation}
    \label{eq:overall_system_1}
    \begin{aligned}
        \dot x
        ={}&f(x)+g(x)\Big[
            \dot{\hat v}+a\omega\cos(\omega t)+\lambda\hat v+\lambda a\sin(\omega t)
        \Big],\\
        \dot{\hat v}
        ={}&-KJ\big(t,h(x)\big)\sin(\omega t).
    \end{aligned}
\end{equation}

The term $a\omega\cos(\omega t)$ has an amplitude that grows with $\omega$ for fixed $a$, so \eqref{eq:overall_system_1} is not in a form ready for averaging analysis. We therefore first apply a coordinate transformation generated by the flow of $g$ to remove this term.








\subsection{Coordinate Transformation}

Consider differential equation $ \frac{dz}{ds} = g(z)$ with solution $\phi$ such that
\begin{equation}
    \label{eq:g_flow_derivative}
    \frac{\partial \phi}{\partial s} (s, \xi) = g(\phi (s,\xi)),\quad \phi(0,\xi) = \xi.
\end{equation}
Let
\begin{equation}
    s(t) \coloneqq a \sin{\omega t},
    \label{eq:definition_s}
\end{equation}
and define the coordinate transformation:
\begin{equation}
    \label{eq:g_flow_transformation}
    x = \phi(s,\xi).
\end{equation}
By continuity of $g$, for any compact set $\mathcal N \in \mathbb{R}^n$, we can find $\overline{a}>0$ such that $\phi$ is diffeomorphism for all $(s,\xi) \in [-\overline{a}, \overline{a}]\times \mathcal{N}$.

Since for any $\xi \in \mathcal{N}$ and $s,r\in \mathbb{R}$ such that $s+r \in [-\overline{a}, \overline{a}]$
\begin{equation}
    \label{eq:flow_property}
    \phi(s, \phi(r,\xi)) = \phi(s + r, \xi),
\end{equation}
we have $\phi(s,\phi(-s,\xi)) = \phi(0,\xi) = \xi$, and thus the inverse transformation of \eqref{eq:g_flow_transformation} is given by
\begin{equation*}
    \xi = \phi(-s,x).
\end{equation*}
Note that $\xi \rightarrow x$ as $a \rightarrow 0$.

%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%
Differentiating the coordinate transformation \eqref{eq:g_flow_transformation} with respect to time gives
\begin{equation}
    \label{eq:coordinate_transformation_step1}
    \dot{x}
    =
    \nabla_{\xi}\phi(s,\xi)\dot{\xi}
    +
    \frac{\partial \phi}{\partial s}(s,\xi)\dot{s}.
\end{equation}
By substituting \eqref{eq:g_flow_derivative} and $\dot s = a\omega\cos(\omega t)$ into \eqref{eq:coordinate_transformation_step1}, we obtain:
\begin{equation}
    \label{eq:x_dot_transformation}
    \dot{x}
    =
    \nabla_{\xi}\phi(s,\xi)\dot{\xi}
    +
    g(\phi(s,\xi))a\omega\cos(\omega t).
\end{equation}

On the other hand, substituting \eqref{eq:g_flow_transformation} and \eqref{eq:definition_s} into \eqref{eq:overall_system_1} gives
\begin{equation*}
    \begin{aligned}
        \dot{x}
        &=
        f(\phi(s,\xi))
        +
        g(\phi(s,\xi))
        \big(
            \dot{\hat v}
            +
            a\omega\cos(\omega t)
            +
            \lambda\hat v
            +
            \lambda s
        \big).
    \end{aligned}
\end{equation*}
Comparing this equation with \eqref{eq:x_dot_transformation}, the term
$$g(\phi(s,\xi))a\omega\cos(\omega t)$$ cancels out, which yields
\begin{equation}
    \label{eq:xi_intermediate}
    \dot{\xi}
    =
    \left[\nabla_{\xi}\phi(s,\xi)\right]^{-1}
    \left[
    f(\phi(s,\xi))
    +
    g(\phi(s,\xi))
    \big( \dot{\hat v} + \lambda\hat v + \lambda s \big)
    \right]
    .
\end{equation}

Next, we simplify \eqref{eq:xi_intermediate} by showing
\begin{equation*}
    \left(\nabla_{\xi}\phi(s,\xi)\right)^{-1} g(\phi(s,\xi)) = g(\xi).
\end{equation*}

Recall the flow property \eqref{eq:flow_property}, differentiating both sides with respect to $r$ and evaluating at $r=0$ gives
\begin{equation}
    \nabla_{\xi}\phi(s+0,\xi)
    \frac{\partial\phi}{\partial r}(0,\xi)
    =
    \frac{\partial\phi}{\partial r}(s+0,\xi).
\end{equation}
Since
\begin{equation*}
    \frac{\partial\phi}{\partial r}(0,\xi)=g(\xi),
    \qquad
    \frac{\partial\phi}{\partial r}(s,\xi)
    =
    g(\phi(s,\xi)),
\end{equation*}
it follows that
\begin{equation}
    \label{eq:g_flow_pushforward}
    \nabla_{\xi}\phi(s,\xi)g(\xi)
    =
    g(\phi(s,\xi)).
\end{equation}
Since $\phi(-s,\cdot)$ is the inverse of $\phi(s,\cdot)$,
$\nabla_{\xi}\phi(s,\xi)$ is nonsingular wherever the flow is defined.
Hence, \eqref{eq:g_flow_pushforward} implies
\begin{equation*}
    \left[\nabla_{\xi}\phi(s,\xi)\right]^{-1}
    g(\phi(s,\xi))
    =
    g(\xi),
\end{equation*}
and \eqref{eq:xi_intermediate} becomes
\begin{equation}
    \label{eq:xi_dynamics}
    \begin{aligned}
        \dot{\xi}
        &=
        \left[\nabla_{\xi}\phi(s,\xi)\right]^{-1}
        f(\phi(s,\xi))
        +
        g(\xi)
        \big(
            \dot{\hat v}
            +
            \lambda\hat v
            +
            \lambda s
        \big).
    \end{aligned}
\end{equation}

Under the coordinate transformation, the measured output becomes
\begin{equation*}
    y=h(\phi(s,\xi)).
\end{equation*}
Consequently, the extremum-seeking update law is
\begin{equation*}
    \dot{\hat v}
    =
    -KJ\left(t,h(\phi(s,\xi))\right)\sin(\omega t).
\end{equation*}
Together, the overall system after coordinate transformation is given by:
\begin{equation}
    \begin{aligned}
        \dot{\xi}
        &=
        \left[\nabla_{\xi}\phi(s,\xi)\right]^{-1}
        f(\phi(s,\xi))
        +g(\xi)\big(\dot{\hat v}+\lambda\hat v + \lambda s \big),
        \\
        \dot{\hat v}&=-KJ\left(t,h(\phi(s,\xi))\right)\sin(\omega t).
    \end{aligned}
    \label{eq:transformed_system}
\end{equation}

The transformation removes the explicit term whose amplitude grows with $\omega$, and \eqref{eq:transformed_system} is in a standard form suitable for the averaging analysis.

\subsection{Averaged System}

Define
\begin{align}
    F(s,\xi)
    &\coloneqq
    \left[\nabla_\xi\phi(s,\xi)\right]^{-1}
    f(\phi(s,\xi)),
    \label{eq:F_definition}\\
    Q(t,s,\xi)
    &\coloneqq
    J\bigl(t,h(\phi(s,\xi))\bigr)
    =\bigl[h(\phi(s,\xi))-y_d(t)\bigr]^2.
    \label{eq:Q_definition}
\end{align}

The Taylor expansion of \eqref{eq:F_definition} and \eqref{eq:Q_definition} around $s=0$, with integral remainders is given by
\begin{equation}
    \begin{aligned}
        F(s,\xi)
        =&F(0,\xi)
        +s\frac{\partial F}{\partial s}(0,\xi)\\
        & +s^2\int_0^1(1-\tau)
        \frac{\partial^2 F}{\partial s^2}(\tau s,\xi)\,d\tau,
    \end{aligned}
    \label{eq:F_Taylor_expansion}
\end{equation}
and
\begin{equation}
    \begin{aligned}
        Q(t,s,\xi)
        ={}&Q(t,0,\xi)
        +s\frac{\partial Q}{\partial s}(t,0,\xi)+\frac{s^2}{2}
        \frac{\partial^2 Q}{\partial s^2}(t,0,\xi)\\
        &+\frac{s^3}{2}\int_0^1(1-\tau)^2
        \frac{\partial^3 Q}{\partial s^3}(t,\tau s,\xi)\,d\tau.
    \end{aligned}
    \label{eq:Q_Taylor_expansion}
\end{equation}
By definition of $F$ in \eqref{eq:F_definition} and property \eqref{eq:g_flow_derivative}, we have
\begin{equation}
    \begin{aligned}
        F(0,\xi) &= \left[\nabla_{\xi}\phi(0,\xi)\right]^{-1} f(\phi(0,\xi))
        \\
        &=  \left[\nabla_{\xi}\xi\right]^{-1} f(\xi)
        \\
        &= I^{-1}f(\xi)
        \\
        &= f(\xi).
    \end{aligned}
    \label{eq:F_component1}
\end{equation}
Moreover, by property \eqref{eq:g_flow_derivative} (i.e., $\phi(0,\xi)=\xi$),
\begin{equation}
    \begin{aligned}
        Q(t,0,\xi)
        &=\bigl[h(\xi)-y_d(t)\bigr]^2,\\
        \frac{\partial Q}{\partial s}(t,0,\xi)
        &=2\bigl[h(\xi)-y_d(t)\bigr]L_gh(\xi),\\
        \frac{\partial^2 Q}{\partial s^2}(t,0,\xi)
        &=2\bigl[L_gh(\xi)\bigr]^2\\
        &\quad
        +2\bigl[h(\xi)-y_d(t)\bigr]L_g^2h(\xi),
    \end{aligned}
    \label{eq:Q_Taylor_coefficients}
\end{equation}
and,
\begin{equation}
    \begin{aligned}
        \frac{\partial^3 Q}{\partial s^3}(t,s,\xi)
        ={}&6L_gh(\phi(s,\xi))
               L_g^2h(\phi(s,\xi))\\
        &+2\bigl[h(\phi(s,\xi))-y_d(t)\bigr]
               L_g^3h(\phi(s,\xi)).
    \end{aligned}
    \label{eq:Q_third_derivative}
\end{equation}

We take the partial average of
\eqref{eq:transformed_system} over the fast phase
$\theta=\omega t$, holding $t$, $\xi$, and $\hat v$ fixed.
The resulting averaged system is
\begin{equation}
    \begin{aligned}
        \dot{\xi}^{av}
        ={}&
        \frac{1}{2\pi}\int_0^{2\pi}
        F(a\sin\theta,\xi^{av})\,d\theta\\
        &+g(\xi^{av})\Bigg[
        \lambda\hat v^{av}
        -\frac{K}{2\pi}\int_0^{2\pi}
        Q(t,a\sin\theta,\xi^{av})
        \sin\theta\,d\theta
        \Bigg],\\
        \dot{\hat v}^{av}
        ={}&
        -\frac{K}{2\pi}\int_0^{2\pi}
        Q(t,a\sin\theta,\xi^{av})
        \sin\theta\,d\theta.
    \end{aligned}
    \label{eq:partial_averaged_system}
\end{equation}

By \eqref{eq:F_Taylor_expansion}, we have
\begin{equation}
    \frac{1}{2\pi}\int_0^{2\pi}
    F(a\sin\theta,\xi)\,d\theta
    =
    f(\xi)+a^2\Gamma_f(\xi,a),
    \label{eq:F_phase_average}
\end{equation}
where
\begin{equation}
    \begin{aligned}
        \Gamma_f(\xi,a)
        \coloneqq{}&
        \frac{1}{2\pi}\int_0^{2\pi}
        \sin^2\theta
        \int_0^1(1-\tau)\\
        &\qquad{}\times
        \frac{\partial^2 F}{\partial s^2}
        (\tau a\sin\theta,\xi)
        \,d\tau\,d\theta.
    \end{aligned}
    \label{eq:Gamma_f_definition}
\end{equation}

Similarly, by \eqref{eq:Q_Taylor_expansion}, we have
\begin{equation}
    \begin{aligned}
        &\frac{K}{2\pi}\int_0^{2\pi}
        Q(t,a\sin\theta,\xi)\sin\theta\,d\theta\\
        &\qquad=
        \kappa\frac{\partial Q}{\partial s}(t,0,\xi)
        +\kappa a^2\Gamma_v(t,\xi,a),
    \end{aligned}
    \label{eq:Q_phase_average}
\end{equation}
where
\begin{equation}
    \kappa\coloneqq\frac{Ka}{2}.
    \label{eq:kappa_definition}
\end{equation}
and
\begin{equation}
    \begin{aligned}
        \Gamma_v(t,\xi,a)
        \coloneqq{}&
        \frac{1}{2\pi}\int_0^{2\pi}
        \sin^4\theta
        \int_0^1(1-\tau)^2\\
        &\qquad{}\times
        \frac{\partial^3 Q}{\partial s^3}
        (t,\tau a\sin\theta,\xi)
        \,d\tau\,d\theta.
    \end{aligned}
    \label{eq:Gamma_v_definition}
\end{equation}

Let
\begin{equation}
    y^{av}\coloneqq h(\xi^{av}),
    \qquad
    e^{av}\coloneqq y^{av}-y_d(t).
    \label{eq:averaged_output_error}
\end{equation}
By substituting \eqref{eq:F_phase_average} and \eqref{eq:Q_phase_average} into \eqref{eq:partial_averaged_system}, the averaged system is
\begin{subequations}
    \label{eq:averaged_system}
    \begin{align}
        \dot{\xi}^{av}
        ={}&
        f(\xi^{av})+a^2\Gamma_f(\xi^{av},a)
        \nonumber\\
        &+g(\xi^{av})\Big[
        \lambda\hat v^{av}
        -2\kappa e^{av}L_gh(\xi^{av})
        \nonumber\\
        &\hspace{3.5em}
        -\kappa a^2\Gamma_v(t,\xi^{av},a)
        \Big],
        \label{eq:averaged_system_xi}\\
        \dot{\hat v}^{av}
        ={}&
        -2\kappa e^{av}L_gh(\xi^{av})
        -\kappa a^2\Gamma_v(t,\xi^{av},a).
        \label{eq:averaged_system_hat_v}
    \end{align}
\end{subequations}






















\subsection{Byrnes--Isidori Form}

On a coordinate domain $\mathcal U\subseteq\mathbb R^n$, consider a diffeomorphism
\begin{equation}
    \Theta(\xi)
    \coloneqq
    \begin{bmatrix}
        \vartheta(\xi)\\
        h(\xi)
    \end{bmatrix},
    \qquad
    \vartheta:\mathcal U\to\mathbb R^{n-1},
    \label{eq:BI_transformation}
\end{equation}
where
\begin{equation}
    \frac{\partial\vartheta}{\partial\xi}(\xi)g(\xi)=0.
    \label{eq:BI_eta_condition}
\end{equation}
Such coordinates exist locally under Assumption~\ref{assum:Relative_degree}.
Define
\begin{equation}
    \begin{bmatrix}
        \eta^{av}\\
        y^{av}
    \end{bmatrix}
    =
    \Theta(\xi^{av}),
    \qquad
    \xi^{av}=\Theta^{-1}(\eta^{av},y^{av}).
    \label{eq:BI_averaged_coordinates}
\end{equation}

For $(\eta,y)\in\Theta(\mathcal U)$, let
\begin{align}
    q(\eta,y)
    &\coloneqq
    \left.
    \frac{\partial\vartheta}{\partial\xi}(\xi)f(\xi)
    \right|_{\xi=\Theta^{-1}(\eta,y)},
    \label{eq:q_definition}\\
    \ell(\eta,y)
    &\coloneqq
    L_fh\bigl(\Theta^{-1}(\eta,y)\bigr),
    \label{eq:ell_definition}\\
    b(\eta,y)
    &\coloneqq
    L_gh\bigl(\Theta^{-1}(\eta,y)\bigr).
    \label{eq:b_definition}
\end{align}
Define the transformed remainder terms
\begin{equation}
    \begin{aligned}
        r_\eta(\eta,y,a)
        &\coloneqq
        \left.
        a^2\frac{\partial\vartheta}{\partial\xi}(\xi)
        \Gamma_f(\xi,a)
        \right|_{\xi=\Theta^{-1}(\eta,y)},\\
        r_y(\eta,y,a)
        &\coloneqq
        \left.
        a^2\frac{\partial h}{\partial\xi}(\xi)
        \Gamma_f(\xi,a)
        \right|_{\xi=\Theta^{-1}(\eta,y)},\\
        \Delta_v(t,\eta,y,a,\kappa)
        &\coloneqq
        -\kappa a^2
        \Gamma_v\bigl(t,\Theta^{-1}(\eta,y),a\bigr).
    \end{aligned}
    \label{eq:BI_remainder_definitions}
\end{equation}

Differentiating $\eta^{av}=\vartheta(\xi^{av})$ along
\eqref{eq:averaged_system} and using
\eqref{eq:BI_eta_condition} gives
\begin{equation}
    \begin{aligned}
        \dot\eta^{av}
        &=
        \frac{\partial\vartheta}{\partial\xi}(\xi^{av})
        \dot\xi^{av}\\
        &=
        \frac{\partial\vartheta}{\partial\xi}(\xi^{av})
        \Big[f(\xi^{av})+a^2\Gamma_f(\xi^{av},a)\Big]\\
        &=
        q(\eta^{av},y^{av})
        +r_\eta(\eta^{av},y^{av},a).
    \end{aligned}
    \label{eq:BI_eta_derivation}
\end{equation}
Similarly, differentiating $y^{av}=h(\xi^{av})$ yields
\begin{equation}
    \begin{aligned}
        \dot y^{av}
        ={}&
        L_fh(\xi^{av})
        +a^2\frac{\partial h}{\partial\xi}(\xi^{av})
        \Gamma_f(\xi^{av},a)\\
        &+L_gh(\xi^{av})\Big[
        \lambda\hat v^{av}
        -2\kappa e^{av}L_gh(\xi^{av})
        -\kappa a^2\Gamma_v(t,\xi^{av},a)
        \Big].
    \end{aligned}
    \label{eq:BI_y_derivation}
\end{equation}

Therefore, the averaged system in Byrnes--Isidori
coordinates is
\begin{equation}
    \begin{aligned}
        \dot\eta^{av}
        ={}&
        q(\eta^{av},y^{av})
        +r_\eta,\\
        \dot y^{av}
        ={}&
        \ell(\eta^{av},y^{av})
        +\lambda b(\eta^{av},y^{av})\hat v^{av}\\
        &-2\kappa b^2(\eta^{av},y^{av})e^{av} + b(\eta^{av},y^{av})\Delta_v +r_y,\\
        \dot{\hat v}^{av}
        ={}&
        -2\kappa b(\eta^{av},y^{av})e^{av}+\Delta_v,
    \end{aligned}
    \label{eq:averaged_BI_system}
\end{equation}
where $$e^{av}=y^{av}-y_d(t).$$ Consequently, for almost everywhere,
\begin{equation}
    \begin{aligned}
        \dot e^{av}
        ={}&
        -2\kappa b^2(\eta^{av},y^{av})e^{av}
        +\ell(\eta^{av},y^{av}) +\lambda b(\eta^{av},y^{av})\hat v^{av}\\
        & -\dot y_d(t)+b(\eta^{av},y^{av})\Delta_v + r_y.
    \end{aligned}
    \label{eq:averaged_tracking_error_dynamics}
\end{equation}






\subsection{SPES of the Averaged Tracking Error}




\begin{assum}[Bounded internal dynamics]
    \label{assum:internal_dynamics}
    There exist a continuously differentiable, positive definite, radially unbounded function $W:\mathbb R^{n-1}\to\mathbb R_{\geq0}$, a class-$\mathcal K_\infty$ function $\alpha$, a continuous non-decreasing function $\sigma:\mathbb R_{\geq0}\to\mathbb R_{\geq0}$,
    and a constant $c_0\geq0$ such that
    \begin{equation}
        \frac{\partial W}{\partial\eta}(\eta)q(\eta,y)
        \leq
        -\alpha(W(\eta))+\sigma(|y|)+c_0
        \label{eq:internal_dissipation}
    \end{equation}
    for all $(\eta,y)\in\mathbb R^{n-1}\times\mathbb R$.
    $\hfill\triangle$
\end{assum}

\begin{lem}[SPES of the averaged tracking error]
    \label{lem:averaged_tracking_SPAS}
    Suppose Assumptions~\ref{assum:Relative_degree},\ref{assum:Reference_trajectory} and \ref{assum:internal_dynamics} hold and fix $\lambda>0$. The following property holds:

    For any $\Delta_1, \delta_1, \rho>0$, there exist $\kappa^*>0$ and $a^*>0$ such that, for all $\kappa\geq\kappa^*$ and $0<a\leq a^*$,
    every solution of \eqref{eq:averaged_system} with $|(\xi^{av}(t_0),\hat v^{av}(t_0))| \leq \Delta_1$, we have
    \begin{equation}
        |e^{av}(t)|
        \leq
        e^{-\rho(t-t_0)}|e^{av}(t_0)|+\delta_1,
        \qquad t\geq t_0.
        \label{eq:averaged_tracking_SPAS}
    \end{equation}

    $\hfill \square$
\end{lem}




\begin{thm}[SPES of tracking error]
    \label{thm:tracking_SPES_transfer} 
    Assumptions~\ref{assum:Relative_degree},\ref{assum:Reference_trajectory} and \ref{assum:internal_dynamics} hold and fix $\lambda>0$. Suppose $\Theta$ is a global diffeomorphism, then the following property hold:

    For any $\Delta,\delta,\rho>0$, there exist $\kappa^*>0$ and $a^*>0$ such that, for every $\kappa\geq\kappa^*$ and $0<a\leq a^*$, there exist $\omega^*>0$ such that for every $\omega\geq\omega^*$, each solution of
    \eqref{eq:overall_system_1} with $|(x(t_0),\hat v(t_0))|\leq\Delta$ satisfies
    \begin{equation}
        |e(t)| \leq e^{-\rho(t-t_0)}|e(t_0)| +\delta, \qquad t\geq t_0.
        \label{eq:original_tracking_transfer_bound}
    \end{equation}
    $\hfill \square$
\end{thm}










==> Chapters/Proof_of_Theorem_backup.tex <==
The proof of Theorem~\ref{thm:tracking_SPES_transfer} is organised into three lemmas. First, we present a general partial averaging lemma for nonlinear time-varying systems with high-frequency periodic excitation, based on the results of \cite{Teel2003Unified}, without reproducing its proof. Second, we derive the partially averaged closed-loop dynamics in the Byrnes--Isidori coordinates defined by $\bm{\Theta}$ in \eqref{eq:BI_transformation} and establish boundedness and semiglobal practical exponential tracking under Assumption~\ref{assum:Internal_dynamics}. Finally, we apply the partial averaging lemma to transfer the tracking property to the transformed closed-loop system, from which the physical output-tracking guarantee follows.



Consider the nonlinear time-varying system
\begin{equation}
    \dot{\bm z}
    =\bm F(t,\bm z,\omega t),
    \label{eq:general_fast_system}
\end{equation}
where $\bm z\in\mathbb R^m$, $\omega>0$,
and $\bm F$ is $2\pi$-periodic in its
third argument. Define the partially averaged system
\begin{equation}
    \dot{\bar{\bm z}}
    =\bar{\bm F}(t,\bar{\bm z}),
    \label{eq:general_averaged_system}
\end{equation}
where
\begin{equation}
    \bar{\bm F}(t,\bm z)
    \coloneqq
    \frac{1}{2\pi}\int_0^{2\pi}
    \bm F(t,\bm z,\theta)\,d\theta.
    \label{eq:general_partial_average}
\end{equation}

\begin{lem}[Stability under partial averaging]
\label{lem:partial_averaging}
Suppose that $\bm F(t,\bm z,\omega t)$ is
$2\pi$-periodic in the fast time $\omega t$,
uniformly bounded on compact state sets,
and locally Lipschitz in $(t,\bm z)$,
with bounds and Lipschitz constants
independent of the fast ``time'' $\omega t$. Assume that the partially averaged system
\eqref{eq:general_averaged_system} is
uniformly semiglobally practically
asymptotically stable with respect to
a compact target set $\mathcal A$. 
Then, for any prescribed compact set
of initial conditions and any practical
stability tolerance, there exists
$\omega^*>0$ such that, for every
$\omega\geq\omega^*$, the original system
\eqref{eq:general_fast_system} is
semiglobally practically asymptotically
stable with respect to $\mathcal A$.
\end{lem}




As established in Section~3.1, the flow-based coordinate transformation \eqref{eq:flow_transformation} eliminates the explicit high-frequency term in \eqref{eq:closed_loop_system}. We now provide the detailed derivation of the transformed system \eqref{eq:transformed_system}.

\subsection{Coordinate Transformation $\bm{\varphi}(s,\bm{\xi})$ using \eqref{eq:flow_transformation}}
%
%%%%%%%%%%%%%%%%%%%%%%%5
\iffalse
Consider the flow $\bm{\varphi}$ generated by $\bm{g}$, satisfying
\begin{equation}
    \label{eq:g_flow_derivative}
    \frac{\partial\bm{\varphi}}{\partial s}(s,\bm{\xi})
    =\bm{g}\bigl(\bm{\varphi}(s,\bm{\xi})\bigr),
    \qquad
    \bm{\varphi}(0,\bm{\xi})=\bm{\xi}.
\end{equation}
Let
\begin{equation}
    s(t)\coloneqq a\sin(\omega t),
    \label{eq:definition_s}
\end{equation}
and define the coordinate transformation
\begin{equation}
    \bm{x}=\bm{\varphi}(s,\bm{\xi}).
    \label{eq:g_flow_transformation}
\end{equation}
Since $\bm{g}$ is of class $C^2$, for any compact set $\mathcal N\subset\mathbb R^n$, there exists $\overline a>0$ such that the flow is defined on a neighbourhood of $[-\overline a,\overline a]\times\mathcal N$. For each fixed $|s|\leq\overline a$, the map $\bm{\varphi}(s,\cdot)$ is a diffeomorphism onto its image.

The flow identity
\begin{equation}
    \bm{\varphi}\bigl(s,\bm{\varphi}(r,\bm{\xi})\bigr)
    =\bm{\varphi}(s+r,\bm{\xi})
    \label{eq:flow_property}
\end{equation}
holds wherever both sides are defined. Thus, the inverse of \eqref{eq:g_flow_transformation} is
\[
    \bm{\xi}=\bm{\varphi}(-s,\bm{x}).
\]
In particular, $\bm{\xi}\to\bm{x}$ as $a\to0$, uniformly on compact sets.
%
\fi


Differentiating \eqref{eq:flow_transformation}
with respect to time and using
\eqref{eq:flow_definition} gives
\begin{equation}
    \dot{\bm{x}}
    =
    \nabla_{\bm{\xi}}\bm{\varphi}(s,\bm{\xi})
    \dot{\bm{\xi}}
    +
    \bm{g}\bigl(\bm{\varphi}(s,\bm{\xi})\bigr)
    a\omega\cos(\omega t).
    \label{eq:x_dot_transformation}
\end{equation}

Substituting \eqref{eq:flow_transformation}
into \eqref{eq:closed_loop_system} and comparing
with \eqref{eq:x_dot_transformation}, the terms
involving $a\omega\cos(\omega t)$ cancel, yielding
\bea
            \dot{\bm{\xi}}
        =
        \left[\nabla_{\bm{\xi}}
        \bm{\varphi}(s,\bm{\xi})\right]^{-1}
        \left[
        \bm{f}\left(\bm{\varphi}(s,\bm{\xi})\right)+
        \bm{g}\left(\bm{\varphi}(s,\bm{\xi})\right)
        \gamma(\dot{\hat v},\hat v, s)
        \right], \hspace{0.3in}
        \label{eq:xi_intermediate}
\eea
where 
\beas 
%
\gamma(\dot{\hat v},\hat v,s)=\dot{\hat v}+\hat v+s.
\eeas
According to \eqref{eq:flow_definition}, the flow generated by $\bm{g}$ satisfies
the composition property
\begin{equation}
    \bm{\varphi}\bigl(s,\bm{\varphi}(r,\bm{\xi})\bigr)
    =
    \bm{\varphi}(s+r,\bm{\xi}),
    \label{eq:flow_property}
\end{equation}
wherever both sides are defined.
Differentiating with respect to $r$ at $r=0$
and using \eqref{eq:flow_definition} yields
\begin{equation}
    \nabla_{\bm{\xi}}\bm{\varphi}(s,\bm{\xi})
    \bm{g}(\bm{\xi})
    =
    \bm{g}\bigl(\bm{\varphi}(s,\bm{\xi})\bigr).
    \label{eq:g_flow_pushforward}
\end{equation}

Since $\nabla_{\bm{\xi}}\bm{\varphi}(s,\bm{\xi})$
is nonsingular, substituting
\eqref{eq:g_flow_pushforward} into
\eqref{eq:xi_intermediate} yields
\eqref{eq:transformed_system}. In the transformed coordinates, define the tracking error as
\begin{equation}
    e_\xi \coloneqq h(\bm{\xi}) - y_d.
    \label{eq:e_xi}
\end{equation}
For small dither amplitudes $a$, this error approximates the physical tracking error $e=h(\bm{x})-y_d$ since $\bm{\xi}\to\bm{x}$ as $a\to0$.
\todo[inline]{}
\subsection{Byrnes--Isidori Coordinate Transformation}
\label{sec:BI_before_averaging}

We now express the transformed closed-loop system
\eqref{eq:transformed_system} in Byrnes--Isidori
coordinates before applying partial averaging.
For convenience, define
\begin{equation}
    \bm f_1(s,\bm\xi)
    \coloneqq
    \bigl[
        \nabla_{\bm\xi}\bm\varphi(s,\bm\xi)
    \bigr]^{-1}
    \bm f\bigl(\bm\varphi(s,\bm\xi)\bigr),
    \label{eq:f1_definition}
\end{equation}
and
\begin{equation}
    \begin{aligned}
        \mathcal J(t,s,\bm\xi)
        &\coloneqq
        J\bigl(t,h(\bm\varphi(s,\bm\xi))\bigr)\\
        &=
        \bigl[
            h(\bm\varphi(s,\bm\xi))-y_d(t)
        \bigr]^2.
    \end{aligned}
    \label{eq:transformed_objective_definition}
\end{equation}
With this notation,
\eqref{eq:transformed_system} becomes
\begin{equation}
    \begin{aligned}
        \dot{\bm\xi}
        ={}&
        \bm f_1(s,\bm\xi)
        +\bm g(\bm\xi)
        \bigl(\dot{\hat v}+\hat v+s\bigr),\\
        \dot{\hat v}
        ={}&
        -K\mathcal J(t,s,\bm\xi)\sin(\omega t),
    \end{aligned}
    \label{eq:transformed_system_compact}
\end{equation}
where $s=a\sin(\omega t)$.

Apply the global coordinate transformation
$\bm\Theta$ in \eqref{eq:BI_transformation},
specified in Assumption~\ref{assum:Internal_dynamics},
to the $\bm \varphi$-transformed state $\bm\xi$:
\begin{equation}
    \begin{bmatrix}
        \bm\eta\\
        y_\xi
    \end{bmatrix}
    =
    \bm\Theta(\bm\xi)
    =
    \begin{bmatrix}
        \bm\vartheta(\bm\xi)\\
        h(\bm\xi)
    \end{bmatrix}.
    \label{eq:BI_transformed_coordinates}
\end{equation}
Here, $y_\xi$ denotes the $\bm \Theta$-transformed output, which is exactly the same as $\bm \varphi$-transformed output $h(\xi)$. Thus the transformed tracking error is still \eqref{eq:e_xi}.


Define the phase-dependent functions
\begin{equation}
    \begin{aligned}
        \bm q_s(\bm\eta,y_\xi)
        \coloneqq{}&
        \left.
        \frac{\partial\bm\vartheta}{\partial\bm\xi}
        (\bm\xi)\bm f_1(s,\bm\xi)
        \right|_{\bm\xi=
        \bm\Theta^{-1}(\bm\eta,y_\xi)},\\
        \ell_s(\bm\eta,y_\xi)
        \coloneqq{}&
        \left.
        \frac{\partial h}{\partial\bm\xi}
        (\bm\xi)\bm f_1(s,\bm\xi)
        \right|_{\bm\xi=
        \bm\Theta^{-1}(\bm\eta,y_\xi)}.
    \end{aligned}
    \label{eq:BI_phase_dependent_drifts}
\end{equation}
%
Since $\bm\varphi(0,\bm\xi)=\bm\xi$ and
$\nabla_{\bm\xi}\bm\varphi(0,\bm\xi)=I$,
\eqref{eq:F_definition} gives
\begin{equation}
    \bm f_1(0,\bm\xi)=\bm f(\bm\xi).
    \label{eq:f_1 property}
\end{equation}
Therefore,
\begin{equation}
    \begin{aligned}
        \bm q_0(\bm\eta,y_\xi)
        &=\bm q(\bm\eta,y_\xi),\\
        \ell_0(\bm\eta,y_\xi)
        &=\ell(\bm\eta,y_\xi),
    \end{aligned}
    \label{eq:BI_zero_phase_drifts}
\end{equation}
where $\bm q$ and $\ell$ come from \eqref{eq:q_definition} and \eqref{eq:ell_definition}, respectively.

Differentiating
$\bm\eta=\bm\vartheta(\bm\xi)$ along
\eqref{eq:transformed_system_compact}
and using \eqref{eq:BI_eta_condition_x} gives
\bea
    \dot{\bm\eta}
    &=&
    \frac{\partial\bm\vartheta}{\partial\bm\xi}
    (\bm\xi)\dot{\bm\xi}
    \nonumber\\
    &=&
    \frac{\partial\bm\vartheta}{\partial\bm\xi}
    (\bm\xi)\bm f_1(s,\bm\xi)
    + \frac{\partial\bm\vartheta}{\partial\bm\xi}
    (\bm\xi)\bm g(\bm\xi)
    \bigl(\dot{\hat v}+\hat v+s\bigr)
    \nonumber\\
    &=&
    \bm q_s(\bm\eta,y_\xi).
    \label{eq:BI_unaveraged_internal_derivation}
\eea
Similarly, differentiating $y_\xi=h(\bm\xi)$ yields
\bea
    \dot y_\xi
    &=&
    \frac{\partial h}{\partial\bm\xi}
    (\bm\xi)\dot{\bm\xi}
    \nonumber\\
    &=&
    \frac{\partial h}{\partial\bm\xi}
    (\bm\xi)\bm f_1(s,\bm\xi)
    +
    L_{\bm g}h(\bm\xi)
    \bigl(\dot{\hat v}+\hat v+s\bigr)
    \nonumber\\
    &=&
    \ell_s(\bm\eta,y_\xi)
    +b(\bm\eta,y_\xi)
    \bigl(\dot{\hat v}+\hat v+s\bigr),
    \label{eq:BI_unaveraged_output_derivation}
\eea
where $b$ is defined in \eqref{eq:b_definition}.

Substituting the controller dynamics \eqref{eq:transformed_system_compact} into
\eqref{eq:BI_unaveraged_output_derivation},
the transformed closed-loop system in
Byrnes--Isidori coordinates is
\begin{equation}
    \begin{aligned}
        \dot{\bm\eta}
        ={}&
        \bm q_s(\bm\eta,y_\xi),\\
        \dot y_\xi
        ={}&
        \ell_s(\bm\eta,y_\xi)
        +b(\bm\eta,y_\xi)(\hat v+s)\\
        &-
        Kb(\bm\eta,y_\xi)
        \mathcal J(t,s,\bm\xi)\sin(\omega t),\\
        \dot{\hat v}
        ={}&
        -K\mathcal J(t,s,\bm\xi)\sin(\omega t),
    \end{aligned}
    \label{eq:unaveraged_BI_system}
\end{equation}
where
$\bm\xi=\bm\Theta^{-1}(\bm\eta,y_\xi)$
and $s=a\sin(\omega t)$.
Equation~\eqref{eq:unaveraged_BI_system}
is an exact coordinate representation of
\eqref{eq:transformed_system}.
The functions $\bm q_s$, $\ell_s$, and
$\mathcal J(t,s,\bm\xi)$ retain their dependence
on the fast phase through $s$.

Finally, since $y_d$ is absolutely continuous under Assumption~\ref{assum:Reference_trajectory}, differentiating \eqref{eq:e_xi} gives
\begin{equation}
    \begin{aligned}
        \dot e_\xi
        ={}&
        \ell_s(\bm\eta,y_\xi)
        +b(\bm\eta,y_\xi)(\hat v+s)\\
        &-
        Kb(\bm\eta,y_\xi)
        \mathcal J(t,s,\bm\xi)\sin(\omega t)
        -\dot y_d(t).
    \end{aligned}
    \label{eq:unaveraged_BI_error_dynamics}
\end{equation}




\subsection{Partially Averaged System}
\label{sec:partial_averaging_BI}

We now apply partial averaging to the
Byrnes--Isidori system
\eqref{eq:unaveraged_BI_system}, following the
framework of \cite{Teel2003Unified}.
The averaging is performed over the fast phase
$\theta=\omega t$, holding
$t$, $\bm\eta$, $y_\xi$, and $\hat v$ fixed. For convenience, define
\bea
    \langle P\rangle_\theta
    &\coloneqq&
    \frac{1}{2\pi}
    \int_0^{2\pi}P(\theta)\,d\theta.
    \label{eq:phase_average_definition}
\eea

We first calculate the averages of $\bm q_s$ and $\ell_s$.
Expanding $\bm f_1(s,\bm\xi)$ about $s=0$ using Taylor's theorem with integral remainder
gives
\bea
    \bm f_1(s,\bm\xi)
    &=&
    \bm f(\bm\xi)
    +s\frac{\partial\bm f_1}{\partial s}
    (0,\bm\xi)
    \nonumber\\
    &&
    {}+s^2\int_0^1(1-\tau)
    \frac{\partial^2\bm f_1}{\partial s^2}
    (\tau s,\bm\xi)\,d\tau,
    \label{eq:F_Taylor_expansion}
\eea
where we have used $\bm f_1(0,\bm\xi)=\bm f(\bm\xi)$.
Define
\bea
    \bm\Gamma_f(\bm\xi,a)
    &\coloneqq&
    \frac{1}{2\pi}
    \int_0^{2\pi}\sin^2\theta
    \int_0^1(1-\tau)
    \nonumber\\
    &&
    {}\times
    \frac{\partial^2\bm f_1}{\partial s^2}
    (\tau a\sin\theta,\bm\xi)
    \,d\tau\,d\theta.
    \label{eq:Gamma_f_definition}
\eea

Since the coordinate transformation
$\bm\Theta$ is independent of the fast phase,
the derivatives
$\partial\bm\vartheta/\partial\bm\xi$
and $\partial h/\partial\bm\xi$
are fixed during averaging.
Using
$\langle\sin\theta\rangle_\theta=0$,
multiplication of
\eqref{eq:F_Taylor_expansion}
by these derivatives yields
\bea
    \bigl\langle
        \bm q_{a\sin\theta}(\bm\eta,y_\xi)
    \bigr\rangle_\theta
    &=&
    \bm q(\bm\eta,y_\xi)+\bm r_\eta,
    \nonumber\\
    \bigl\langle
        \ell_{a\sin\theta}(\bm\eta,y_\xi)
    \bigr\rangle_\theta
    &=&
    \ell(\bm\eta,y_\xi)+r_y,
    \label{eq:BI_averaged_drift_terms}
\eea
where
\bea
    \bm r_\eta(\bm\eta,y_\xi,a)
    &\coloneqq&
    a^2
    \frac{\partial\bm\vartheta}{\partial\bm\xi}
    (\bm\xi)\bm\Gamma_f(\bm\xi,a),
    \nonumber\\
    r_y(\bm\eta,y_\xi,a)
    &\coloneqq&
    a^2
    \frac{\partial h}{\partial\bm\xi}
    (\bm\xi)\bm\Gamma_f(\bm\xi,a).
    \label{eq:BI_drift_remainder_definitions}
\eea
Next, we calculate the averaged controller dynamics. Taylor expansion of $\mathcal J(t,s,\bm\xi)$ about $s=0$
gives
\bea
    \mathcal J(t,s,\bm\xi)
    &=&
    \mathcal J(t,0,\bm\xi)
    +s\frac{\partial\mathcal J}{\partial s}
    (t,0,\bm\xi)+\frac{s^2}{2}
    \frac{\partial^2\mathcal J}{\partial s^2}
    (t,0,\bm\xi)
    \nonumber\\
    &&
    {}+\frac{s^3}{2}
    \int_0^1(1-\tau)^2
    \frac{\partial^3\mathcal J}{\partial s^3}
    (t,\tau s,\bm\xi)\,d\tau.
    \label{eq:Q_Taylor_expansion}
\eea
By the definition of $\mathcal J$ and the
flow equation \eqref{eq:flow_definition},
\bea
    \mathcal J(t,0,\bm\xi)
    &=&
    \bigl[h(\bm\xi)-y_d(t)\bigr]^2
    =e_\xi^2,
    \nonumber\\
    \frac{\partial\mathcal J}{\partial s}
    (t,0,\bm\xi)
    &=&
    2\bigl[h(\bm\xi)-y_d(t)\bigr]
    L_{\bm g}h(\bm\xi)
    \nonumber\\
    &=&
    2e_\xi b(\bm\eta,y_\xi).
    \label{eq:Q_derivative_at_zero}
\eea
The higher derivatives in
\eqref{eq:Q_Taylor_expansion} exist under the
assumed regularity of $\bm g$ and $h$.

Substituting $s=a\sin\theta$ into
\eqref{eq:Q_Taylor_expansion},
multiplying by $\sin\theta$, and using
\bea
    \langle\sin\theta\rangle_\theta
    &=&
    \langle\sin^3\theta\rangle_\theta=0,
    \nonumber\\
    \langle\sin^2\theta\rangle_\theta
    &=&
    \frac12,
    \label{eq:phase_sine_moments}
\eea
gives
\bea
    &&
    \bigl\langle
        \mathcal J(t,a\sin\theta,\bm\xi)
        \sin\theta
    \bigr\rangle_\theta
    \nonumber\\
    &=&
    \frac a2
    \frac{\partial\mathcal J}{\partial s}
    (t,0,\bm\xi)
    +\frac{a^3}{2}\Gamma_v(t,\bm\xi,a),
    \label{eq:Q_phase_average}
\eea
where
\bea
    \Gamma_v(t,\bm\xi,a)
    &\coloneqq&
    \frac{1}{2\pi}
    \int_0^{2\pi}\sin^4\theta
    \int_0^1(1-\tau)^2
    \nonumber\\
    &&
    {}\times
    \frac{\partial^3\mathcal J}{\partial s^3}
    (t,\tau a\sin\theta,\bm\xi)
    \,d\tau\,d\theta.
    \label{eq:Gamma_v_definition}
\eea

Using the effective gain $\kappa=Ka/2$,
equations
\eqref{eq:Q_derivative_at_zero}
and \eqref{eq:Q_phase_average}
yield
\bea
    &&
    \bigl\langle
        -K\mathcal J(t,a\sin\theta,\bm\xi)
        \sin\theta
    \bigr\rangle_\theta
    \nonumber\\
    &=&
    -\kappa
    \frac{\partial\mathcal J}{\partial s}
    (t,0,\bm\xi)
    -\kappa a^2\Gamma_v(t,\bm\xi,a)
    \nonumber\\
    &=&
    -2\kappa b(\bm\eta,y_\xi)e_\xi+r_v,
    \label{eq:BI_controller_phase_average}
\eea
where
\bea
    r_v(t,\bm\eta,y_\xi,a,\kappa)
    &\coloneqq&
    -\kappa a^2
    \Gamma_v(t,\bm\xi,a),
    \label{eq:BI_controller_remainder}
\eea
with
$\bm\xi=\bm\Theta^{-1}(\bm\eta,y_\xi)$.
Moreover, $b(\bm\eta,y_\xi)$ is independent
of the fast phase at the fixed state, so
\bea
    \bigl\langle
        b(\bm\eta,y_\xi)a\sin\theta
    \bigr\rangle_\theta
    &=&
    0.
    \label{eq:BI_additive_dither_average}
\eea

The remainder functions admit uniform bounds
on compact state sets.
Indeed, let $\mathcal P$ be a compact set in
$(\bm\eta,y_\xi)$ coordinates and define
$\mathcal N=\bm\Theta^{-1}(\mathcal P)$.
Choose $\bar a>0$ sufficiently small that
the flow is defined on a neighbourhood of
$[-\bar a,\bar a]\times\mathcal N$.
The derivatives appearing in
\eqref{eq:Gamma_f_definition}
and \eqref{eq:Gamma_v_definition}
are bounded there, uniformly in $t$,
because $|y_d(t)|\leq R$.
The coordinate derivatives are also bounded
on $\mathcal N$.
Consequently, there exists $C>0$,
independent of $t$, $a$, and $\kappa$,
such that
\bea
    \|\bm r_\eta(\bm\eta,y_\xi,a)\|
    +|r_y(\bm\eta,y_\xi,a)|
    &\leq&
    Ca^2,
    \nonumber\\
    |r_v(t,\bm\eta,y_\xi,a,\kappa)|
    &\leq&
    C\kappa a^2
    \label{eq:BI_remainder_bounds}
\eea
for all $(\bm\eta,y_\xi)\in\mathcal P$,
$t\geq0$, $0<a\leq\bar a$, and $\kappa>0$.

Denote the averaged state by
$(\bm\eta^{av},y_\xi^{av},\hat v^{av})$,
and define
\bea
    \bm\xi^{av}
    &\coloneqq&
    \bm\Theta^{-1}(\bm\eta^{av},y_\xi^{av}).
    \label{eq:averaged_state_reconstruction}
\eea
The averaged tracking error is
\bea
    e_\xi^{av}
    &\coloneqq&
    y_\xi^{av}-y_d(t)
    \nonumber\\
    &=&
    h(\bm\xi^{av})-y_d(t).
    \label{eq:e_xi_av}
\eea

Combining
\eqref{eq:BI_averaged_drift_terms},
\eqref{eq:BI_controller_phase_average},
and \eqref{eq:BI_additive_dither_average},
the partially averaged system associated
with \eqref{eq:unaveraged_BI_system} is
\bea
    \dot{\bm\eta}^{av}
    &=&
    \bm q(\bm\eta^{av},y_\xi^{av})
    +\bm r_\eta,
    \nonumber\\
    \dot y_\xi^{av}
    &=&
    \ell(\bm\eta^{av},y_\xi^{av})
    +b(\bm\eta^{av},y_\xi^{av})\hat v^{av}
    \nonumber\\
    &&
    {}-2\kappa
    b^2(\bm\eta^{av},y_\xi^{av})e_\xi^{av}
    \nonumber\\
    &&
    {}+b(\bm\eta^{av},y_\xi^{av})r_v+r_y,
    \nonumber\\
    \dot{\hat v}^{av}
    &=&
    -2\kappa
    b(\bm\eta^{av},y_\xi^{av})e_\xi^{av}
    +r_v,
    \label{eq:averaged_BI_system}
\eea
where the remainder terms are evaluated along
the averaged trajectory:
\beas
    \bm r_\eta
    &=&
    \bm r_\eta(\bm\eta^{av},y_\xi^{av},a),\\
    r_y
    &=&
    r_y(\bm\eta^{av},y_\xi^{av},a),\\
    r_v
    &=&
    r_v(t,\bm\eta^{av},y_\xi^{av},a,\kappa).
\eeas

Finally, differentiating
\eqref{eq:e_xi_av} and using
\eqref{eq:averaged_BI_system}
gives, for almost every $t$ in the
interval of existence,
\bea
    \dot e_\xi^{av}
    &=&
    -2\kappa
    b^2(\bm\eta^{av},y_\xi^{av})e_\xi^{av}
    \nonumber\\
    &&
    {}+\ell(\bm\eta^{av},y_\xi^{av})
    +b(\bm\eta^{av},y_\xi^{av})\hat v^{av}
    \nonumber\\
    &&
    {}-\dot y_d(t)
    +b(\bm\eta^{av},y_\xi^{av})r_v+r_y,
    \label{eq:averaged_BI_error_dynamics}
\eea
where $y_\xi^{av}=e_\xi^{av}+y_d(t)$.







\todo[inline]{}
\subsection{Averaged System}

We now apply partial averaging to the transformed closed-loop system \eqref{eq:transformed_system}, following the framework of \cite{Teel2003Unified}, to characterise the effective dynamics induced by the high-frequency dither.

{\bf Weixuan, I want you to take over the proof.

We now analyse the stability of the partially averaged closed-loop system \eqref{eq:transformed_system}. Applying the Byrnes--Isidori coordinate transformation $\bm{\Theta}$ in
    \eqref{eq:BI_transformation}, we first establish boundedness of the averaged closed-loop trajectories and then derive a practical exponential tracking estimate using Lyapunov analysis.

I want to introduce $e^{\bm{\xi}}$ at the beginning, and re-write \eqref{eq:transformed_system} into new coordinate. Then directly apply partial averaging. 


}




Using \eqref{eq:flow_transformation} and
\eqref{eq:tracking_objective}, define
\bea
\bm{f_1}(s,\bm{\xi})
&\coloneqq&
\bigl[\nabla_{\bm{\xi}}\bm{\varphi}(s,\bm{\xi})\bigr]^{-1}
\bm{f}\bigl(\bm{\varphi}(s,\bm{\xi})\bigr),
\label{eq:F_definition}
\eea
Expanding $\bm{f_1}(\cdot,\cdot)$ in \eqref{eq:F_definition}
about $s=0$ using Taylor's theorem with
integral remainder yields
\begin{equation}
\begin{aligned}
\bm{f_1}(s,\bm{\xi})
={}&\bm{f_1}(0,\bm{\xi})
+s\frac{\partial\bm{f_1}}{\partial s}(0,\bm{\xi})\\
&+s^2\int_0^1(1-\tau)
\frac{\partial^2\bm{f_1}}{\partial s^2}
(\tau s,\bm{\xi})\,d\tau.
\end{aligned}
\label{eq:F_Taylor_expansion}
\end{equation}
By \eqref{eq:F_definition} and \eqref{eq:flow_definition}, it has
\[
    \bm{f_1}(0,\bm{\xi})=\bm{f}(\bm{\xi}).
\]
For simplicity, we write 
\begin{equation}
    J(t,s,\bm \xi) = J(t, h(\bm \varphi (s,\bm \xi))),
\end{equation}
we have
\begin{equation}
    \begin{aligned}
        J(t,s,\bm{\xi})
        ={}&J(t,0,\bm{\xi})
        +s\frac{\partial J}{\partial s}(t,0,\bm{\xi})\\
        &+\frac{s^2}{2}\frac{\partial^2 J}{\partial s^2}(t,0,\bm{\xi})\\
        &+\frac{s^3}{2}\int_0^1(1-\tau)^2
        \frac{\partial^3 J}{\partial s^3}(t,\tau s,\bm{\xi})\,d\tau,
    \end{aligned}
    \label{eq:Q_Taylor_expansion}
\end{equation}
where $J(t,0,\bm{\xi})=\bigl[h(\bm{\xi})-y_d(t)\bigr]^2$, $\frac{\partial J}{\partial s}(t,0,\bm{\xi})
        =2\bigl[h(\bm{\xi})-y_d(t)\bigr]L_{\bm{g}}h(\bm{\xi})$, and the expressions of $\frac{\partial^2 J}{\partial s^2}(t,0,\bm{\xi})$ and $\frac{\partial^3 J}{\partial s^3}(t,s,\bm{\xi})$ are omitted here.
% \beas
%        &\ & J(t,0,\bm{\xi})
%         =\bigl[h(\bm{\xi})-y_d(t)\bigr]^2,\\
%         &\ & \frac{\partial J}{\partial s}(t,0,\bm{\xi})
%         =2\bigl[h(\bm{\xi})-y_d(t)\bigr]L_{\bm{g}}h(\bm{\xi}),\\
%         &\ & \frac{\partial^2 J}{\partial s^2}(t,0,\bm{\xi})
%         =2\bigl[L_{\bm{g}}h(\bm{\xi})\bigr]^2+2\bigl[h(\bm{\xi})-y_d(t)\bigr]L_{\bm{g}}^2h(\bm{\xi}),
% \eeas
% and
% \[
%     \begin{aligned}
%         \frac{\partial^3 J}{\partial s^3}(t,s,\bm{\xi})
%         ={}&6L_{\bm{g}}h\bigl(\bm{\varphi}(s,\bm{\xi})\bigr)
%         L_{\bm{g}}^2h\bigl(\bm{\varphi}(s,\bm{\xi})\bigr)\\
%         &+2\bigl[h(\bm{\varphi}(s,\bm{\xi}))-y_d(t)\bigr]\\
%         &\quad\times L_{\bm{g}}^3h\bigl(\bm{\varphi}(s,\bm{\xi})\bigr).
%     \end{aligned}
% \]

We partially average \eqref{eq:transformed_system} over the fast phase $\theta=\omega t$, holding $t$, $\bm{\xi}$, and $\hat v$ fixed. Using \eqref{eq:F_Taylor_expansion} and \eqref{eq:Q_Taylor_expansion}, the resulting system can be written as
\begin{equation}
    \begin{aligned}
        \dot{\bm{\xi}}^{av}
        ={}&\bm{f}(\bm{\xi}^{av})+a^2\bm{\Gamma}_f(\bm{\xi}^{av},a)\\
        &+\bm{g}(\bm{\xi}^{av})\Big[
        \hat v^{av}-2\kappa e^{av}L_{\bm{g}}h(\bm{\xi}^{av})\\
        &\hspace{6em}-\kappa a^2\Gamma_v(t,\bm{\xi}^{av},a)
        \Big],\\
        \dot{\hat v}^{av}
        ={}&-2\kappa e^{av}L_{\bm{g}}h(\bm{\xi}^{av})
        -\kappa a^2\Gamma_v(t,\bm{\xi}^{av},a),
    \end{aligned}
    \label{eq:averaged_system}
\end{equation}
where
\begin{equation}
    e^{av}\coloneqq y^{av}-y_d(t)
    \label{eq:e_av}
\end{equation}
and the remainder functions are defined by
\[
    \begin{aligned}
        \bm{\Gamma}_f(\bm{\xi},a)
        \coloneqq{}&
        \frac{1}{2\pi}\int_0^{2\pi}
        \sin^2\theta\int_0^1(1-\tau)\\
        &\quad\times
        \frac{\partial^2\bm{f_1}}{\partial s^2}
        (\tau a\sin\theta,\bm{\xi})
        \,d\tau\,d\theta,\\
        \Gamma_v(t,\bm{\xi},a)
        \coloneqq{}&
        \frac{1}{2\pi}\int_0^{2\pi}
        \sin^4\theta\int_0^1(1-\tau)^2\\
        &\quad\times
        \frac{\partial^3 J}{\partial s^3}
        (t,\tau a\sin\theta,\bm{\xi})
        \,d\tau\,d\theta.
    \end{aligned}
\]










% This gives
% \begin{equation}
%     \begin{aligned}
%         \dot{\bm{\xi}}^{av}
%         ={}&\frac{1}{2\pi}\int_0^{2\pi}
%         \bm{f_1}(a\sin\theta,\bm{\xi}^{av})\,d\theta\\
%         &+\bm{g}(\bm{\xi}^{av})\Bigg[
%         \hat v^{av}\\
%         &\qquad-\frac{K}{2\pi}\int_0^{2\pi}
%         J(t,a\sin\theta,\bm{\xi}^{av})\sin\theta\,d\theta
%         \Bigg],\\
%         \dot{\hat v}^{av}
%         ={}&-\frac{K}{2\pi}\int_0^{2\pi}
%         J(t,a\sin\theta,\bm{\xi}^{av})\sin\theta\,d\theta.
%     \end{aligned}
%     \label{eq:partial_averaged_system}
% \end{equation}
% By \eqref{eq:F_Taylor_expansion},
% \begin{equation}
%     \frac{1}{2\pi}\int_0^{2\pi}
%     \bm{f_1}(a\sin\theta,\bm{\xi})\,d\theta
%     =\bm{f}(\bm{\xi})+a^2\bm{\Gamma}_f(\bm{\xi},a),
%     \label{eq:F_phase_average}
% \end{equation}
% where
% \[
%     \begin{aligned}
%         \bm{\Gamma}_f(\bm{\xi},a)
%         \coloneqq{}&\frac{1}{2\pi}\int_0^{2\pi}
%         \sin^2\theta\int_0^1(1-\tau)\\
%         &\qquad\times\frac{\partial^2\bm{f_1}}{\partial s^2}
%         (\tau a\sin\theta,\bm{\xi})\,d\tau\,d\theta.
%     \end{aligned}
% \]
% Similarly, \eqref{eq:Q_Taylor_expansion} gives
% \begin{equation}
%     \begin{aligned}
%         &\frac{K}{2\pi}\int_0^{2\pi}
%         J(t,a\sin\theta,\bm{\xi})\sin\theta\,d\theta\\
%         &\qquad=\kappa\frac{\partial J}{\partial s}(t,0,\bm{\xi})
%         +\kappa a^2\Gamma_v(t,\bm{\xi},a),
%     \end{aligned}
%     \label{eq:Q_phase_average}
% \end{equation}
% where $\kappa\coloneqq Ka/2$ and
% \[
%     \begin{aligned}
%         \Gamma_v(t,\bm{\xi},a)
%         \coloneqq{}&\frac{1}{2\pi}\int_0^{2\pi}
%         \sin^4\theta\int_0^1(1-\tau)^2\\
%         &\qquad\times\frac{\partial^3 J}{\partial s^3}
%         (t,\tau a\sin\theta,\bm{\xi})\,d\tau\,d\theta.
%     \end{aligned}
% \]

% Let
% \[
%     y^{av}\coloneqq h(\bm{\xi}^{av}),
%     \qquad
%     e^{av}\coloneqq y^{av}-y_d(t).
% \]
% Substituting \eqref{eq:F_phase_average} and \eqref{eq:Q_phase_average} into \eqref{eq:partial_averaged_system} yields
% \begin{equation}
%     \begin{aligned}
%         \dot{\bm{\xi}}^{av}
%         ={}&\bm{f}(\bm{\xi}^{av})+a^2\bm{\Gamma}_f(\bm{\xi}^{av},a)\\
%         &+\bm{g}(\bm{\xi}^{av})\Big[
%         \hat v^{av}-2\kappa e^{av}L_{\bm{g}}h(\bm{\xi}^{av})\\
%         &\hspace{6em}-\kappa a^2\Gamma_v(t,\bm{\xi}^{av},a)
%         \Big],\\
%         \dot{\hat v}^{av}
%         ={}&-2\kappa e^{av}L_{\bm{g}}h(\bm{\xi}^{av})
%         -\kappa a^2\Gamma_v(t,\bm{\xi}^{av},a).
%     \end{aligned}
%     \label{eq:averaged_system}
% \end{equation}

\subsection{Byrnes--Isidori Form}

Apply the global coordinate transformation $\bm{\Theta}$ in \eqref{eq:BI_transformation}, specified in Assumption~\ref{assum:Internal_dynamics}, to the averaged state $\bm{\xi}^{av}$:
\[
    \begin{bmatrix}
        \bm{\eta}^{av}\\
        y^{av}
    \end{bmatrix}
    =\bm{\Theta}(\bm{\xi}^{av}),
    \qquad
    \bm{\xi}^{av}=\bm{\Theta}^{-1}(\bm{\eta}^{av},y^{av}).
\]
The functions $\bm{q}$, $\ell$, and $b$ retain their definitions in \eqref{eq:q_definition}--\eqref{eq:b_definition}. Define the transformed remainder terms
\begin{equation}
    \begin{aligned}
        \bm{r}_\eta(\bm{\eta},y,a)
        &\coloneqq\left.
        a^2\frac{\partial\bm{\vartheta}}{\partial\bm{\xi}}(\bm{\xi})
        \bm{\Gamma}_f(\bm{\xi},a)
        \right|_{\bm{\xi}=\bm{\Theta}^{-1}(\bm{\eta},y)},\\
        r_y(\bm{\eta},y,a)
        &\coloneqq\left.
        a^2\frac{\partial h}{\partial\bm{\xi}}(\bm{\xi})
        \bm{\Gamma}_f(\bm{\xi},a)
        \right|_{\bm{\xi}=\bm{\Theta}^{-1}(\bm{\eta},y)},\\
        r_v(t,\bm{\eta},y,a,\kappa)
        &\coloneqq-\kappa a^2
        \Gamma_v\bigl(t,\bm{\Theta}^{-1}(\bm{\eta},y),a\bigr).
    \end{aligned}
    \label{eq:BI_remainder_definitions}
\end{equation}

Differentiating $\bm{\eta}^{av}=\bm{\vartheta}(\bm{\xi}^{av})$ along \eqref{eq:averaged_system} and using \eqref{eq:BI_eta_condition_x} gives
\[
    \begin{aligned}
        \dot{\bm{\eta}}^{av}
        &=\frac{\partial\bm{\vartheta}}{\partial\bm{\xi}}(\bm{\xi}^{av})
        \dot{\bm{\xi}}^{av}\\
        &=\frac{\partial\bm{\vartheta}}{\partial\bm{\xi}}(\bm{\xi}^{av})
        \Big[\bm{f}(\bm{\xi}^{av})+a^2\bm{\Gamma}_f(\bm{\xi}^{av},a)\Big]\\
        &=\bm{q}(\bm{\eta}^{av},y^{av})
        +\bm{r}_\eta(\bm{\eta}^{av},y^{av},a).
    \end{aligned}
\]
Similarly, differentiating $y^{av}=h(\bm{\xi}^{av})$ yields
\[
    \begin{aligned}
        \dot y^{av}
        ={}&L_{\bm{f}}h(\bm{\xi}^{av})
        +a^2\frac{\partial h}{\partial\bm{\xi}}(\bm{\xi}^{av})
        \bm{\Gamma}_f(\bm{\xi}^{av},a)\\
        &+L_{\bm{g}}h(\bm{\xi}^{av})\Big[
        \hat v^{av}-2\kappa e^{av}L_{\bm{g}}h(\bm{\xi}^{av})\\
        &\hspace{6em}-\kappa a^2\Gamma_v(t,\bm{\xi}^{av},a)
        \Big].
    \end{aligned}
\]
Therefore, the averaged system in Byrnes--Isidori coordinates is
\begin{equation}
    \begin{aligned}
        \dot{\bm{\eta}}^{av}
        ={}&\bm{q}(\bm{\eta}^{av},y^{av})+\bm{r}_\eta,\\
        \dot y^{av}
        ={}&\ell(\bm{\eta}^{av},y^{av})
        +b(\bm{\eta}^{av},y^{av})\hat v^{av}\\
        &-2\kappa b^2(\bm{\eta}^{av},y^{av})e^{av}
        +b(\bm{\eta}^{av},y^{av})r_v+r_y,\\
        \dot{\hat v}^{av}
        ={}&-2\kappa b(\bm{\eta}^{av},y^{av})e^{av}+r_v,
    \end{aligned}
    \label{eq:averaged_BI_system}
\end{equation}
where the remainder terms are evaluated along the averaged trajectory and $e^{av}$ is defined in \eqref{eq:e_av}. Consequently, for almost every $t\geq t_0$,
\[
    \begin{aligned}
        \dot e^{av}
        ={}&-2\kappa b^2(\bm{\eta}^{av},y^{av})e^{av}
        +\ell(\bm{\eta}^{av},y^{av})\\
        &+b(\bm{\eta}^{av},y^{av})\hat v^{av}-\dot y_d(t)\\
        &+b(\bm{\eta}^{av},y^{av})r_v+r_y.
    \end{aligned}
\]

\begin{lem}[SPES of the averaged tracking error]
    \label{lem:averaged_tracking_SPAS}
    Suppose Assumptions~\ref{assum:Relative_degree}--\ref{assum:Reference_trajectory} hold. For any $\Delta^{av},\delta^{av},\rho>0$, there exist $\kappa^*>0$ and $a^*>0$ such that, for all $\kappa\geq\kappa^*$ and $0<a\leq a^*$, every solution of \eqref{eq:averaged_system} with $|(\bm{\xi}^{av}(t_0),\hat v^{av}(t_0))|\leq\Delta^{av}$ is forward complete and satisfies
    \begin{equation}
        |e^{av}(t)|
        \leq\exp\bigl(-\rho(t-t_0)\bigr)|e^{av}(t_0)|+\delta^{av},
        \qquad t\geq t_0.
        \label{eq:averaged_tracking_SPAS}
    \end{equation}
    \hfill$\square$
\end{lem}

Lemma~\ref{lem:partial_averaging} and Lemma~\ref{lem:averaged_tracking_SPAS} together prove the following Proposition.
\begin{prop}[SPES of $e_\xi$]
    \label{prop:SPES_of_e_xi}
    Suppose Assumptions~\ref{assum:Relative_degree}--\ref{assum:Reference_trajectory} hold. For any $\Delta_\xi,\delta_\xi,\rho_\xi>0$, there exist $\kappa_\xi^*>0$ and $a_\xi^*>0$ such that, for all $\kappa\geq\kappa_\xi^*$ and $0<a\leq a_\xi^*$, there exists $\omega^*>0$ such that, for every $\omega\geq\omega^*$, every solution of \eqref{eq:transformed_system} with $|(\bm{\xi}(t_0),\hat v(t_0))|\leq\Delta_\xi$ is forward complete and satisfies
    \begin{equation}
        |e_\xi(t)|
        \leq\exp\bigl(-\rho_\xi(t-t_0)\bigr)|e_\xi(t_0)|+\delta_\xi,
        \qquad t\geq t_0.
        \label{eq:shifted_system_SPAS}
    \end{equation}
    \hfill$\square$
\end{prop}

Fix $\Delta,\rho,\delta>0$. For all sufficiently small $a$, \eqref{eq:inverse_flow_transformation} maps $|(\bm{x}(t_0),\hat v(t_0))|\leq\Delta$ into $|(\bm{\xi}(t_0),\hat v(t_0))|\leq\Delta_\xi$ for a fixed $\Delta_\xi>0$, uniformly in $t_0$ and $\omega$. Apply Proposition~\ref{prop:SPES_of_e_xi} with $\rho_\xi=\rho$ and $\delta_\xi=\delta/2$.

On the common compact neighbourhood obtained in the proof of Proposition~\ref{prop:SPES_of_e_xi}, smoothness of $h$ and $\bm{\varphi}$ gives
\[
    \begin{aligned}
        |e(t)-e_\xi(t)|
        &=\bigl|h\bigl(\bm{\varphi}(a\sin(\omega t),\bm{\xi}(t))\bigr)
        -h(\bm{\xi}(t))\bigr|\\
        &\leq C_ha,
    \end{aligned}
\]
where $C_h>0$ is independent of $\kappa$, $a$, and $\omega$. Reduce the amplitude threshold so that $C_ha\leq\delta/4$. For every admissible $\kappa,a$ and sufficiently large $\omega$, Proposition~\ref{prop:SPES_of_e_xi} then yields
\[
    \begin{aligned}
        |e(t)|
        &\leq e^{-\rho(t-t_0)}|e_\xi(t_0)|
        +\frac{\delta}{2}+C_ha\\
        &\leq e^{-\rho(t-t_0)}|e(t_0)|
        +\frac{\delta}{2}+2C_ha\\
        &\leq e^{-\rho(t-t_0)}|e(t_0)|+\delta,
        \qquad t\geq t_0.
    \end{aligned}
\]
The coordinate transformation also gives forward completeness of the original closed-loop system. This proves Theorem~\ref{thm:tracking_SPES_transfer}.
\hfill$\blacksquare$
